ReconBoost: Boosting Can Achieve Modality Reconcilement

This paper explores a novel multi-modal alternating learning paradigm pursuing a reconciliation between the exploitation of uni-modal features and the exploration of cross-modal interactions. This is motivated by the fact that current paradigms of multi-modal learning tend to explore multi-modal features simultaneously. The resulting gradient prohibits further exploitation of the features in the weak modality, leading to modality competition, where the dominant modality overpowers the learning process. To address this issue, we study the modality-alternating learning paradigm to achieve reconcilement. Specifically, we propose a new method called ReconBoost to update a fixed modality each time. Herein, the learning objective is dynamically adjusted with a reconcilement regularization against competition with the historical models. By choosing a KL-based reconcilement, we show that the proposed method resembles Friedman's Gradient-Boosting (GB) algorithm, where the updated learner can correct errors made by others and help enhance the overall performance. The major difference with the classic GB is that we only preserve the newest model for each modality to avoid overfitting caused by ensembling strong learners. Furthermore, we propose a memory consolidation scheme and a global rectification scheme to make this strategy more effective. Experiments over six multi-modal benchmarks speak to the efficacy of the method. We release the code at https://github.com/huacong/ReconBoost.

==> sec/discard.tex <==
\newpage
% \section{Understanding \name from the perspective of features learning}

% \begin{lemma}
%     [The Relationship between the Feature Quality and the Performance of the Approach] The performance of training with different modality modulation strategies is related to its ability to learn latent features.
% \end{lemma}

% \begin{proof}
%      Assuming that we have obtained encoders $\varphi_1,\varphi_2$ and classifier $W_1, W_2$, with different modality-learning methods. Then, according to \cite{nips21-multi}, for all $0<\delta<1$, with probability at least $1-\frac{\delta}{2}$:
%      \begin{align}
%          & r(W_1\circ \varphi_1) - r(W_2\circ \varphi_2) \\
%          & \le \gamma_{S}(\varphi_1,\varphi_2) + 8L\Re(\mathcal{W}\circ \Phi) + \frac{4C}{\sqrt{m}} + 2C\sqrt{\frac{2\ln(2/\delta)}{m}}
%      \end{align}
%      $\gamma_{S}(\varphi_1,\varphi_2)$ measures the difference of the latent feature quality between different modality learning methods.
% \end{proof}


% \begin{theorem}
%     [Modality Reconcilement] For a specific modality $\mathcal{X}$, during uni-modal training, it will learn $U$ features (denoted as $\{\varphi_{\mathcal{X},i}^{uni}\}_{i=1}^{U}$, with decreasing order of predicting probability $\{p_{\mathcal{X},i}^{uni}\}_{i=1}^{U}$). In the naive approach, it will learn $N$ features (denoted as $\{\varphi_{\mathcal{X},i}^{naive}\}_{i=1}^{N}$, with decreasing order of predicting probability  $\{p_i^{naive}\}_{i=1}^{N}$). With the \name method, it will learn $R$ features (denoted as $\{\varphi_{\mathcal{X},i}^{Recon}\}_{i=1}^{R}$, with decreasing order of predicting probability $\{p_{\mathcal{X},i}^{Recon}\}_{i=1}^{R}$). We have that:
%     \begin{itemize}
%         \item \textbf{Quantity:}$R > U >N$
%         \item \textbf{Quality:} $\sum_{i=1}^{R}p_{\mathcal{X},i}^{Recon} > \sum_{i=1}^{U}p_{\mathcal{X},i}^{uni} > \sum_{i=1}^{N}p_{\mathcal{X},i}^{naive}$
%     \end{itemize}    
% \end{theorem}


% \begin{proof}
%     In uni-modal training, modality $\mathcal{X}_1$ and modality $\mathcal{X}_2$ learn the following features respectively.
%     \begin{align}
%         \mathcal{X}_1: \{\varphi_{\mathcal{X}_1,1}^{Uni},\varphi_{\mathcal{X}_1,2}^{Uni},\cdots,\varphi_{\mathcal{X}_1,U_1}^{Uni}\} \\
%         \mathcal{X}_2: \{\varphi_{\mathcal{X}_2,1}^{Uni},\varphi_{\mathcal{X}_2,2}^{Uni},\cdots,\varphi_{\mathcal{X}_2,U_2}^{Uni}\}
%     \end{align}
%     In naive multi-modal training, modality $\mathcal{X}_1$ and modality $\mathcal{X}_2$ learn the following features.
%     \begin{align}
%         \mathcal{X}_1: \{\varphi_{\mathcal{X}_1,1}^{Naive},\varphi_{\mathcal{X}_1,2}^{Naive},\cdots,\varphi_{\mathcal{X}_1,K_1}^{Naive},\varphi_{\mathcal{X}_1,K_1+1}^{Naive},\cdots,\varphi_{\mathcal{X}_1,N_1}^{Naive}\} \\
%         \mathcal{X}_2: \{\varphi_{\mathcal{X}_2,1}^{Naive},\varphi_{\mathcal{X}_2,2}^{Naive},\cdots,\varphi_{\mathcal{X}_2,K_2}^{Naive},\varphi_{\mathcal{X}_2,K_2+1}^{Naive},\cdots,\varphi_{\mathcal{X}_2,N_2}^{Naive}\}
%     \end{align}

% Among them, the features that can be learned by relying on the uni-modality are as follows:
% \begin{align}
%     \mathcal{X}_1: \{\varphi_{\mathcal{X}_1,1}^{Naive},\varphi_{\mathcal{X}_1,2}^{Naive},\cdots,\varphi_{\mathcal{X}_1,K_1}^{Naive}\} = \{\varphi_{\mathcal{X}_1,1}^{Uni},\varphi_{\mathcal{X}_1,2}^{Uni},\cdots,\varphi_{\mathcal{X}_1,K_1}^{Uni}\} 
%     \label{equ:x1_single}
%     \\
%     \mathcal{X}_2: \{\varphi_{\mathcal{X}_2,1}^{Naive},\varphi_{\mathcal{X}_2,2}^{Naive},\cdots,\varphi_{\mathcal{X}_2,K_2}^{Naive}\} = \{\varphi_{\mathcal{X}_2,1}^{Uni},\varphi_{\mathcal{X}_2,2}^{Uni},\cdots,\varphi_{\mathcal{X}_2,K_2}^{Uni}\}
%     \label{equ:x2_single}
% \end{align}
% where $K_1 < U_1$ and $K_2 < U_2$. The fact that two feature sets are the same means that every corresponding feature in the two feature sets is the same. In the feature set learned by naive multi-modal, in addition to the features that can be obtained by independent learning (Eq.\eqref{equ:x1_single} and Eq.\eqref{equ:x2_single}), there are also the following features:
% \begin{align}
%     \mathcal{X}_1: \{\varphi_{\mathcal{X}_1,K_1+1}^{Naive},\varphi_{\mathcal{X}_1,2}^{Naive},\cdots,\varphi_{\mathcal{X}_1,N_1}^{Naive}\}
%     \\
%     \mathcal{X}_2:\{\varphi_{\mathcal{X}_2,K_2+1}^{Naive},\varphi_{\mathcal{X}_2,2}^{Naive},\cdots,\varphi_{\mathcal{X}_2,N_2}^{Naive}\}
% \end{align}
% where these features are learned by cross-modality learning. 



% For the modality $\mathcal{X}_1$, we have:
% \begin{align}
%     p_{\mathcal{X}_1,K_1+1}^{Uni} > p_{\mathcal{X}_1,K_1+1}^{Naive}  
% \end{align}
% If not, in uni-modal learning, the modality $\mathcal{X}_1$ would learn $\varphi_{\mathcal{X}_1, K_1+1}^{Naive}$ instead of $\varphi_{\mathcal{X}_1,K_1+1}^{Uni}$ which will increase the predicting probability of each data point.

% So, it is obvious that,
% \begin{align}
%     p_{\mathcal{X}_1,U_1}^{Uni} > p_{\mathcal{X}_1,K_1+1}^{Naive}
% \end{align}
% According to \cite{UMT}, we have $U_1 > N_1$. So, 
% \begin{align}
%     \sum_{i=1}^{U_1} p_{\mathcal{X}_1, i}^{Uni} > \sum_{i=1}^{N_1} p_{\mathcal{X}_1, i}^{Naive}
% \end{align}
% The similar conclusion can be drawn for modality $\mathcal{X}_2$:
% \begin{align}
%     \sum_{i=1}^{U_2} p_{\mathcal{X}_2, i}^{Uni} > \sum_{i=1}^{N_1} p_{\mathcal{X}_1, i}^{Naive}
% \end{align}
% In \name training, modality $\mathcal{X}_1$ and modality $\mathcal{X}_2$ learn the following features.
% \begin{align}
%     \mathcal{X}_1: \{\varphi_{\mathcal{X}_1,1}^{Recon},\varphi_{\mathcal{X}_1,2}^{Recon},\cdots,\varphi_{\mathcal{X}_1,N_1}^{Recon},\varphi_{\mathcal{X}_1,N_1+1}^{Recon},\cdots,\varphi_{\mathcal{X}_1,R_1}^{Recon}\} \\
%     \mathcal{X}_1: \{\varphi_{\mathcal{X}_2,1}^{Recon},\varphi_{\mathcal{X}_2,2}^{Recon},\cdots,\varphi_{\mathcal{X}_2,N_2}^{Recon},\varphi_{\mathcal{X}_2,N_2+1}^{Recon},\cdots,\varphi_{\mathcal{X}_2,R_2}^{Recon}\}
% \end{align}
% From the perspective of feature learning, we can divide the ReconBoost learning method into three phases:
% \begin{itemize}
%     \item \textbf{Phase 1:} Inherit features from naive multi-modal learning.
%     \item \textbf{Phase 2:} Learning the uni-modal features that were not captured in naive multi-modal learning.
%     \item \textbf{Phase 3:} Learning multi-modal residual equivalent features.
% \end{itemize}

% \textbf{Initialization} At the initial stage, the feature set for modality $i$, learned using the \name method, is defined as $\Phi_i = \varnothing$.

% \begin{figure*}[h]
%     \centering
%     \includegraphics[width=0.9\linewidth]{icml2024/figure/phase0.png}
%     \caption{The visualization of learned features at the initial stage. }
%     \label{fig:phase0}
% \end{figure*}

% \textbf{Phase 1:  Inherit features from naive multi-modal learning.} 

% As \name is a form of multi-modal learning, it inherits features from naive multi-modal learning. 

% Therefore,
% \begin{align}
%     \mathcal{X}_1:  \Phi_1 = \{\varphi_{\mathcal{X}_1,1}^{Naive},\varphi_{\mathcal{X}_1,2}^{Naive},\cdots,\varphi_{\mathcal{X}_1,N_1}^{Naive}\} \subset
%     \{\varphi_{\mathcal{X}_1,1}^{Recon},\varphi_{\mathcal{X}_1,2}^{Recon},\cdots,\varphi_{\mathcal{X}_1,R_1}^{Recon}\}
%     \\
%     \mathcal{X}_2: \Phi_2 =
%     \{\varphi_{\mathcal{X}_2,1}^{Naive},\varphi_{\mathcal{X}_2,2}^{Naive},\cdots,\varphi_{\mathcal{X}_2,N_2}^{Naive}\} \subset
%     \{\varphi_{\mathcal{X}_2,1}^{Recon},\varphi_{\mathcal{X}_2,2}^{Recon},\cdots,\varphi_{\mathcal{X}_2,N_1}^{Recon}\}
% \end{align}
%  After Phase 1, the visualization of learned features is depicted in the Figure\ref{fig:phase1}.
 
% \begin{figure*}[htbp]
%     \centering
%     \includegraphics[width=0.9\linewidth]{icml2024/figure/phase1.png}
%     \caption{The visualization of learned features after Phase 1. }
%     \label{fig:phase1}
% \end{figure*}

% \textbf{Phase 2: Learning the uni-modal features that were not captured in naive multi-modal learning.} 

% In the proposed \name method, upon the introduction of a modality $\mathcal{X}_1$, according to the optimization objective of the proposed method, one component is to minimize:
% \begin{align}
%     \mathcal{L}(h(\mathcal{X}_1),Y)
%     \label{equ:phase2_ori_obj}
% \end{align}
% where $h$ is the predictor comprising both an encoder and a classifier.

% According to the Lemma \ref{lemma1}, assuming that we can find the best classifier for each feature in the feature set, we can formulate an equivalent expression for the optimization objective, formally as:
% \begin{align}
%     \mathcal{L}(h(\mathcal{X}_1),Y) \equiv   \sum_{\varphi_{i}\in \Phi_i}\ell(f\circ \varphi_{i}) \equiv   \sum_{i=1}^{N_1} p_{\mathcal{X}_1,i}^{Naive}
%     \label{equ:phase2_obj}
% \end{align}
% On the left-hand side, we measure the model performance, while on the right-hand side, we assess the quality of features. We have established a connection between the two through Lemma\ref{lemma1}. 

% Now, we are at the end of Phase 1, and Phase 2 will be dedicated to  minimize the first term, which is equivalent to obtaining more powerful features. 

% Since this process relies solely on uni-modal learning, it will result in the acquisition of more powerful uni-modal features. \textbf{With the gradient descent algorithm for optimization, the model will learn the most powerful uni-modal feature to accelerate the convergence of the objective function.}

% In addition to the feature set $\Phi_1$, we add the most powerful uni-modal feature $\varphi_{\mathcal{X}_1,K_1+1}^{Uni}$. \textbf{$\varphi_{\mathcal{X}_1,K_1+1}^{Uni}$ is the most powerful uni-modal feature for $\mathcal{X}_1$, because it has been chosen in uni-modal learning after $\varphi_{\mathcal{X}_1,K_1}^{Uni}$}. Similar, for modality $\mathcal{X}_2$, we add the most powerful uni-modal feature $\varphi_{\mathcal{X}_1,K_2+1}^{Uni}$ in $\Phi_2$. After several iterations, we get:
% \begin{align}
%      \mathcal{X}_1:  \Phi_1 = \{\varphi_{\mathcal{X}_1,1}^{Naive},\varphi_{\mathcal{X}_1,2}^{Naive},\cdots,\varphi_{\mathcal{X}_1,N_1}^{Naive},\varphi_{\mathcal{X}_1,K_1+1}^{Uni},\cdots,\varphi_{\mathcal{X}_1,U_1}^{Uni}\} \subset
%     \{\varphi_{\mathcal{X}_1,1}^{Recon},\varphi_{\mathcal{X}_1,2}^{Recon},\cdots,\varphi_{\mathcal{X}_1,R_1}^{Recon}\}
%     \\
%     \mathcal{X}_2: \Phi_2 =
%     \{\varphi_{\mathcal{X}_2,1}^{Naive},\varphi_{\mathcal{X}_2,2}^{Naive},\cdots,\varphi_{\mathcal{X}_2,N_2}^{Naive},\varphi_{\mathcal{X}_2,K_2+1}^{Uni},\cdots,\varphi_{\mathcal{X}_2,U_2}^{Uni}\} \subset
%     \{\varphi_{\mathcal{X}_2,1}^{Recon},\varphi_{\mathcal{X}_2,2}^{Recon},\cdots,\varphi_{\mathcal{X}_2,N_1}^{Recon}\}
% \end{align}

%  After Phase 2, the visualization of learned features is depicted in the Figure\ref{fig:phase2}.
 
% \begin{figure*}[htbp]
%     \centering
%     \includegraphics[width=0.9\linewidth]{icml2024/figure/phase2.png}
%     \caption{The visualization of learned features after Phase 2. }
%     \label{fig:phase2}
% \end{figure*}


% \textbf{Phase 3: Learning multi-modal residual equivalent features.}

% Let $\mathcal{C}_1$ and $\mathcal{C}_2$ be the complete feature sets for modalities $\mathcal{X}_1$ and $\mathcal{X}_2$, respectively.

% The optimization objective $\mathcal{L}\left(h_1(\mathcal{X}_1), - \nabla L (h_2(\mathcal{X}_2) , \mathcal{Y} ) \right)$ of the proposed \name can be equivalently written as:
% \begin{align}
%     \mathcal{L}\left(h_1(\mathcal{X}_1), - \nabla L (h_2(\mathcal{X}_2) , \mathcal{Y} ) \right) \equiv \sum_{\varphi_{\mathcal{X}_1,i}\in \Phi_1,\varphi_{\mathcal{X}_2,j}^{Res}\in (\mathcal{C}_2 - \Phi_2)} \ell(f_1^{*}\circ\varphi_{\mathcal{X}_1,i}, f_2^{*}\circ \varphi_{\mathcal{X}_2,j}^{Res})
% \end{align}

% To minimize the objective function, optimization of the feature set $\Phi_1$ is necessary. For modality $\mathcal{X}_1$, we aim to learn a set of equivalent features denoted as $\{\varphi_{\mathcal{X}_1,r}^{Eqv}\}_{r=1}^{V_1}$ that correspond to residual features in modality $\mathcal{X}_2$, ensuring that $\ell(f_1^{*}\circ\varphi_{\mathcal{X}_1,r}^{Eqv}, f_2^{*}\circ \varphi_{\mathcal{X}_2,j}^{Res})$  is minimized. Since $\varphi_{\mathcal{X}_2,j}^{Res}$ contributes positively to the overall logits, $\{\varphi_{\mathcal{X}_1,r}^{Eqv}\}_{r=1}^{V_1}$ also has a positive impact on the logits, implying that $\sum_{r = 1}^{V}p_{\mathcal{X}_1,r}^{Eqv} > 0$. According to the definition of cross-modal features, these features for modality $\mathcal{X}_1$ belong to the cross-modal feature set. After several iterations, we get:
% \begin{align}
%     \mathcal{X}_1: \Phi_1 = \{\varphi_{\mathcal{X}_1,1}^{Naive},\varphi_{\mathcal{X}_1,2}^{Naive},\cdots,\varphi_{\mathcal{X}_1,N_1}^{Naive},\varphi_{\mathcal{X}_1,K_1+1}^{Uni},\cdots,\varphi_{\mathcal{X}_1,U_1}^{Uni},\varphi_{\mathcal{X}_1,1}^{Eqv},\cdots,\varphi_{\mathcal{X}_1,V_1}^{Eqv}\} = \{\varphi_{\mathcal{X}_1,1}^{Recon},\cdots,\varphi_{\mathcal{X}_1,R_1}^{Recon}\} \\
% \end{align}
% where $R_1 = N_1 + (U_1 - K_1) + V_1$. It's obvious that:
% \begin{align}
%     & \textbf{Quantity}\quad R_1 > U_1 > N_1 \\
%     & \textbf{Quality}\quad \sum_{i=1}^{R}p_{\mathcal{X}_1,i}^{Recon} > \sum_{i=1}^{U}p_{\mathcal{X}_1,i}^{uni} > \sum_{i=1}^{N}p_{\mathcal{X}_1,i}^{naive}
% \end{align}

%  After Phase 3, the visualization of learned features is depicted in the Figure\ref{fig:phase3}.
% \begin{figure*}[htbp]
%     \centering
%     \includegraphics[width=0.9\linewidth]{icml2024/figure/phase3.png}
%     \caption{The visualization of learned features after Phase 3. }
%     \label{fig:phase3}
% \end{figure*}

% \end{proof}


